Learning State Conditioned Linear Mappings for Low-Dimensional Control of Robotic Manipulators

Identifying an appropriate task space that simplifies control solutions is important for solving robotic manipulation problems. One approach to this problem is learning an appropriate low-dimensional action space. Linear and nonlinear action mapping methods have trade-offs between simplicity on the one hand and the ability to express motor commands outside of a single low-dimensional subspace on the other. We propose that learning local linear action representations that adapt based on the current configuration of the robot achieves both of these benefits. Our state-conditioned linear maps ensure that for any given state, the high-dimensional robotic actuations are linear in the low-dimensional action. As the robot state evolves, so do the action mappings, ensuring the ability to represent motions that are immediately necessary. These local linear representations guarantee desirable theoretical properties by design, and we validate these findings empirically through two user studies. Results suggest state-conditioned linear maps outperform conditional autoencoder and PCA baselines on a pick-and-place task and perform comparably to mode switching in a more complex pouring task.

==> exp_subsec/human_reversibility.tex <==
\subsection{Human reversibility}

system is only trained to go from A to B, not B to A, with our system it is easy to go back and forth. 


\textbf{Hypotehsis}: Our system will be able to go from A to B and B to A because of our provable reversibility but AE method will not (ideally). PCA might come close / be comparable.

\paragraph{HOw do we do data collection}
Kinesthetic demonstrations - so we just generate some data on the task of going from A to B. 


\paragraph{evaluation}
invite people (ideally at least 10??) to try 3 different trained systems on collected data
\begin{enumerate}
    \item PCA
    \item AE
    \item Our method
\end{enumerate}

\paragraph{ranking tasks}

\begin{enumerate}
    \item reach from point A to point B amount of sample 
    \item Reach from point A on table to point B on high shelf
    \item moving a long a line but ONLY showing moving in 1 direction 
\end{enumerate}
\paragraph{metrics}
\begin{enumerate}
    \item time to complete task
    \item success: A to B within some distance euclidean distance of end effector or L2 of joints to target config. 
    \item measure joint distance from original $s_{0}$ to $s_{T}$ after returning to point A  ideally $s_{0} \approx s_{T}$
\end{enumerate}

==> exp_subsec/including_task_info_sim.tex <==
\subsection{Affects of including Task Information}

One limitation of our method is that a realistic use case might be only having a single DOF for control. This would limit any actions along a single degree of control. This suggests that being able to then have additional information is a necessity to compenstate for the lack of DOFs. 

To demonstrate this limitation, we train a SCL map with a single DOF with and with-out task specific information.

\paragraph{Reaching} Our first version of this experiment considers a reaching task where we include the desired target as part of the state $s = [q, x, y]$. We then choose an action of $z = 0.5$  and attempt to reach to each point in the validation set. We repeat 5 times. 

We train with $Lipschitz = 0.999$ and do not orthonormalize the vectors in this experiment. 
\textbf{Hypothesis} \textit{When trained without the task information the SCL map will be less effective at reaching the points on the line}

\textbf{Metrics}
\begin{itemize}
    \item Average final distance to target point 
\end{itemize}

As our other point is to maximize control, we compare against a black box AE as well to demonstrate the advantage of the intuitive control. 

\textbf{Hypothesis} \textit{When trained as a black box auto-encoder, the model will move towards the target even when $z = 0$}

To test this, we simply set z = 0 and visualize the results over 10 times steps comparing the SCL map to a vanilla AE model. 

\vz{caveat} hm...I wonder if including target in the encoder will change AE results. it would make sense if it did. maybe z = 0 will be more intuitive at that point. Guess we shall see


include more features?

hack our way to good performance :D 
\begin{itemize}
    \item over complete information
    \item end-effector (- target)
    \item distance metric?
\end{itemize}


Try also 2D z? - idea is again... how well can we reach target but not clear. generalization of method. 

different training data per target, generalization. 

more interesting is generalization to new provided target. seemed to kinda do... 



==> exp_subsec/latent_scalability_sim.tex <==
\subsection{Scalability of Latent Actions}
In this section, we are interested in probing the latent action space to determine whether the property of scalability is achieved in an end-to-end system with our model.
To test for this, we use an adjoint method where we seek to find the latent action $z$ that maps to our target action $a^{*}$
\begin{equation}
    \min_{z} ||a^{*} - \hat{a}||^{2}_{2}
\end{equation}
We do this by gradient descent for our method and an end-to-end auto-encoder model methods. 

With this in mind, we seek to test the following hyptotheses:
\begin{itemize}
    \item \textbf{Hypothesis 1}: the latent action's $z$ will lead to magnitude of actions that correspond to the size of $z$ where the end-to-end model will not give this behavior. 
    \item \textbf{Hypothesis 2}: When given task specific actions, both our model and the end-to-end model will recover the actions
    \item \textbf{Question 3}: Can our trained models capture the underlying task specific action? test with Adjoint method.
\end{itemize}

To test Hypothesis one, we are interested to compare for starting at $z = 0$ whether the scaling action is reachable under the end-to-end model and our own model. so whether for $\alpha \in (-1, 1), \min_{z} ||\alpha g(s, 0) - g(s, 0)||^{2}_{2}$. 

As an argument can be made that an end-to-end system is not trained for this purpose, we also consider finding latent action's $z$ for actions that are produced by the underlying control policy and how these are mapped in the latent space. 



==> exp_subsec/lipschitz_check.tex <==
\subsection{Lipschitz Constraint}

In this experiment, we are interested in checking if training with the Lipschitz regularizer of \cite{gouk2020regularisation} works in our context. To check this, we train our system with and without Gram-Schmidt orthogonality. We use a training and validation set from our task of reaching to a line. 

To verify the Lipschitz constant, we sample random pairs of states and check the Lipschitz Criteria for the chosen constant we train with. 

\paragraph{Hypothesis}
When training with the regularize of \cite{gouk2020regularisation} we expect our model to explicitly maintain the lipschitz constraint for any pairs of data points whether using our orthonormalization or not. 

We look at Root MSE on the validation set in Table~\ref{tab:lipschitz} and show the variability of the Linear mapping predictions in Figure~\ref{fig:lipschitzcheck}.

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\begin{tabular}{@{}lll@{}}
\toprule
\multicolumn{1}{c}{Decoder Training Parameters}                             & \multicolumn{1}{c}{RMSE} & \multicolumn{1}{c}{$\%$ Lipschitz} \\ \midrule
No Lipschitz, No Orthonormal & $0.00272$      & $58.455  \pm 10.488 $                \\ 
No Lipschitz, Orthonormal    & $0.00248$      & $99.970  \pm 0.059 $                  \\
K = .99, No Orthonormal      & $0.0094$       & $100.0$                \\ 
K = .99,  Orthonormal        & $0.00858$      & $99.762 \pm 0.202$                \\ \bottomrule

\end{tabular}
\centering
\caption{Line Reaching Task. Percentage Lipschitz is proportion of times constraint is held for random pairs of states in validation set. We exclude standard deviation when smaller than 3 decimal places.}
\label{tab:lipschitz}
\end{table}

\begin{figure}
    \centering
    \includegraphics[width=.8\linewidth]{exp_subsec/figures/variability_of_linear_maps_lipschitz.jpg}
    \caption{Checking the variability of of Linear Mapping predictions trained with and without Lipschitz condition and orthogonalization proceedure.}
    \label{fig:lipschitzcheck}
\end{figure}

\begin{algorithm}[]
\SetAlgoLined
\KwData{$g_{\theta}(s)$, $D=\{(s_{i}, i \in \{1,...N\}\}$ (dataset), $p$, $L$}
\KwResult{Whether pair of points is lipschits}

$s \sim D$ \;
$s' \sim D$ \;
%\For{$t\gets0$ \KwTo $...$}{ 
$\text{IsLipschitz} \leftarrow ||g_{\theta}(s) - g_{\theta}(s')||_{p} \leq L||s - s'||_{p}$ \;

 \caption{Check Lipschits condition}
 \label{alg:lipschitzcheck}
\end{algorithm}

==> exp_subsec/reachability_sim.tex <==
\subsection{Reversibility in Simulation}

In this section, we are interested in probing how well our trained models can return to to an initial state $s_{0}$ when an action $z$ moves it to some nearby state. 

To control the distance traveled, we generate $z$ from an Isotropic Gaussian distribution and normalize the action to have unit length one. This allows us to control how large the change in distance will be from the initial state. 

From the generated $s' = s + W(s)z$, we then can use the Normal equations of our linear system to derive inverse actions to return to the original state. We include an outline of the experiment loop in Algorithm~\ref{alg:exploop}.

\textbf{Hypothesis} We suspect that for near by states our model with already converge back to the original state but as we progressively take larger step sizes we will not be able to return

\textbf{metrics}
\begin{itemize}
    \item number of steps to return to original states
    \item average final error
\end{itemize}

\begin{figure}
\begin{subfigure}{.5\textwidth}
  \centering
  % include first image
  \includegraphics[width=.8\linewidth]{exp_subsec/figures/reversibility_error_metric_e_0_logscale_True.jpg}  
  \caption{Initial error when taking actions with $||z||=1$ and scaled by $\alpha$}
  \label{fig:sub-first}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
  \centering
  % include second image
  \includegraphics[width=.8\linewidth]{exp_subsec/figures/reversibility_error_metric_e_T_logscale_True.jpg}  
  \caption{Final Error when attempting to return to original state}
  \label{fig:sub-second}
\end{subfigure}
\caption{}
\label{fig:softreachability}
\end{figure}


\begin{algorithm}[]
\SetAlgoLined
\KwData{$\alpha$, $g_{\theta}(s)$, $s_{0}$}
\KwResult{$e_{T}$, $e_{0}$}

$z \sim N(0, \mathbb{I})$\;
$z \leftarrow \frac{\alpha z}{||z||}$\;
$W \leftarrow g_{\theta}(s)$\;
$s' \leftarrow s + Wz$\;
$e_{0} \leftarrow ||s' - s||$\;
%\For{$t\gets0$ \KwTo $...$}{ 
\While{$||s' - s|| \geq \epsilon$}{
    $\Delta s = s' - s$\;
   $W \leftarrow g_{\theta}(s')$\;
   
   $z' \leftarrow W^{\dagger}\Delta s$\;
   $s' \leftarrow s' + Wz'$\;
}

$e_{T} \leftarrow ||s' -s ||$ \;
 \caption{Soft Reversibility Experiment}
 \label{alg:exploop}
\end{algorithm}

\vz{do proper soft invertibility experiment based on our theory}

==> exp_subsec/training_challenges.tex <==
\subsection{Training Challenges}

\paragraph{what is happening during training??}
A relevant question is to check what are the values of the $z_{a}$ values during training. 



==> experiments.tex <==
\section{Experiments} \label{sec:experiments}

\paragraph{Things to test in simulation}
\begin{itemize}
    \item  Can we solve different tasks? some ideas based on previous work:
    \begin{itemize}
        \item follow a sine wave
        \item move on 2 circles \& move between them
        \item 
    \end{itemize}
    \item are the properties we claiming we get, actually happen?
    
\end{itemize}


\input{exp_subsec/latent_scalability_sim}
\input{exp_subsec/lipschitz_check}
\input{exp_subsec/reachability_sim}
\input{exp_subsec/sample_complexity}
\input{exp_subsec/human_reversibility}
\input{exp_subsec/including_task_info_sim}
\input{exp_subsec/latent_scalability_sim}
\input{exp_subsec/training_challenges}
\input{exp_subsec/user_study}

\paragraph{Things to do in user study}
\begin{itemize}
    \item absolutely no idea
\end{itemize}

\subsection{}


